Strong Lens Models for 37 Clusters of Galaxies from the SDSS Giant Arcs Survey

We present strong gravitational lensing models for 37 galaxy clusters from the SDSS Giant Arcs Survey. We combine data from multi-band Hubble Space Telescope WFC3imaging, with ground-based imaging and spectroscopy from Magellan, Gemini, APO, and MMT, in order to detect and spectroscopically confirm new multiply-lensed background sources behind the clusters. We report spectroscopic or photometric redshifts of sources in these fields, including cluster galaxies and background sources. Based on all available lensing evidence, we construct and present strong lensing mass models for these galaxy clusters.

==> files/1604_ztable.tex <==
& 01:30:58.282 & +00:16:45.00 & 241.0371 & GMOS-GN11AQ19\\ 
& 01:30:57.804 & +00:17:04.18 & 241.0391 & GMOS-GN11AQ19\\ 
& 01:30:57.972 & +00:16:52.86 & 241.0207 & GMOS-GN11AQ19\\ 
& 01:30:57.648 & +00:17:23.80 & 241.0420 & GMOS-GN11AQ19\\ 
& 01:30:56.186 & +00:17:20.25 & 241.0466 & GMOS-GN11AQ19\\ 
& 01:30:54.060 & +00:17:15.71 & 241.0408 & GMOS-GN11AQ19\\ 
& 01:30:57.645 & +00:17:24.00 & 241.0369 & GMOS-GN11AQ19\\ 
& 01:30:57.258 & +00:17:23.70 & 241.0423 & GMOS-GN11AQ19\\ 
& 01:30:56.952 & +00:16:52.69 & 241.0427 & GMOS-GN11AQ19\\ 


==> files/s1100arcs.tex <==
1.1 & 167.581480 & 64.999411 & 2.4810 & & \\ 

